Amplitude analysis and branching fraction measurement of $B^{+}\to D^{*-}D^{+}_{s}\pi^{+}$ decays

The decays of the $B^{+}$ meson to the final state $D^{*-}D^{+}_{s}\pi^{+}$ are studied in proton-proton collision data collected with the LHCb detector at centre-of-mass energies of 7, 8, and 13 TeV, corresponding to a total integrated luminosity of 9 fb$^{-1}$. The ratio of branching fractions of the $B^{+}\to D^{*-}D^{+}_{s}\pi^{+}$ and $B^{0}\to D^{*-}D^{+}_{s}$ decays is measured to be $0.173\pm 0.006\pm 0.010$, where the first uncertainty is statistical and the second is systematic. Using partially reconstructed $D^{*+}_{s}\to D^{+}_{s}\gamma$ and $D^{+}_{s}\pi^{0}$ decays, the ratio of branching fractions between the $B^{+}\to D^{*-}D^{*+}_{s}\pi^{+}$ and $B^{+}\to D^{*-}D^{+}_{s}\pi^{+}$ decays is determined as $1.31\pm 0.07\pm 0.14$. An amplitude analysis of the $B^{+}\to D^{*-}D^{+}_{s}\pi^{+}$ decay is performed for the first time, revealing dominant contributions from known excited charm resonances decaying to the $D^{*-}\pi^{+}$ final state. No significant evidence of exotic contributions in the $D^{+}_{s}\pi^{+}$ or $D^{*-}D^{+}_{s}$ channels is found. The fit fraction of the scalar state $T_{c\bar{s} 0}^{\ast}(2900)^{++}$ observed in the $B^{+}\to D^{-}D^{+}_{s}\pi^{+}$ decay is determined to be less than 2.3% at a 90% confidence level.

==> Authorship_LHCb-PAPER-2024-001-arXiv.tex <==
LHCb collaboration:
R. Aaij,
A.S.W. Abdelmotteleb,
C. Abellan Beteta,
F. Abudin{\'e}n,
T. Ackernley,
A. A.  Adefisoye,
B. Adeva,
M. Adinolfi,
P. Adlarson,
C. Agapopoulou,
C.A. Aidala,
Z. Ajaltouni,
S. Akar,
K. Akiba,
P. Albicocco,
J. Albrecht,
F. Alessio,
M. Alexander,
Z. Aliouche,
P. Alvarez Cartelle,
R. Amalric,
S. Amato,
J.L. Amey,
Y. Amhis,
L. An,
L. Anderlini,
M. Andersson,
A. Andreianov,
P. Andreola,
M. Andreotti,
D. Andreou,
A. Anelli,
D. Ao,
F. Archilli,
M. Argenton,
S. Arguedas Cuendis,
A. Artamonov,
M. Artuso,
E. Aslanides,
M. Atzeni,
B. Audurier,
D. Bacher,
I. Bachiller Perea,
S. Bachmann,
M. Bachmayer,
J.J. Back,
P. Baladron Rodriguez,
V. Balagura,
W. Baldini,
H.  Bao,
J. Baptista de Souza Leite,
M. Barbetti,
I. R. Barbosa,
R.J. Barlow,
M. Barnyakov,
S. Barsuk,
W. Barter,
M. Bartolini,
J. Bartz,
F. Baryshnikov,
J.M. Basels,
G. Bassi,
B. Batsukh,
A. Battig,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I.B. Bediaga,
S. Belin,
V. Bellee,
K. Belous,
I. Belov,
I. Belyaev,
G. Benane,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
S. Bernet Andres,
A. Bertolin,
C. Betancourt,
F. Betti,
J.  Bex,
Ia. Bezshyiko,
J. Bhom,
M.S. Bieker,
N.V. Biesuz,
P. Billoir,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
T. Blake,
F. Blanc,
J.E. Blank,
S. Blusk,
V. Bocharnikov,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A.  Bohare,
A. Boldyrev,
C.S. Bolognani,
R. Bolzonella,
N. Bondar,
F. Borgato,
S. Borghi,
M. Borsato,
J.T. Borsuk,
S.A. Bouchiba,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
M.J. Bradley,
A. Brea Rodriguez,
N. Breer,
J. Brodzicka,
A. Brossa Gonzalo,
J. Brown,
D. Brundu,
E. Buchanan,
A. Buonaura,
L. Buonincontri,
A.T. Burke,
C. Burr,
A. Butkevich,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
S. Calderon Ramirez,
L. Calefice,
S. Cali,
M. Calvi,
M. Calvo Gomez,
J. I. Cambon Bouzas,
P. Campana,
D.H. Campora Perez,
A.F. Campoverde Quezada,
S. Capelli,
L. Capriotti,
R. Caravaca-Mora,
A. Carbone,
L. Carcedo Salgado,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carus,
A. Casais Vidal,
R. Caspary,
G. Casse,
J. Castro Godinez,
M. Cattaneo,
G. Cavallero,
V. Cavallini,
S. Celani,
D. Cervenkov,
S.  Cesare,
A.J. Chadwick,
I. Chahrour,
M. Charles,
Ph. Charpentier,
C.A. Chavez Barajas,
M. Chefdeville,
C. Chen,
S. Chen,
Z. Chen,
A. Chernov,
S. Chernyshenko,
V. Chobanova,
S. Cholak,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
X. Cid Vidal,
G. Ciezarek,
P. Cifra,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
C. Cocha Toapaxi,
V. Coco,
J. Cogan,
E. Cogneras,
L. Cojocariu,
P. Collins,
T. Colombo,
A. Comerma-Montells,
L. Congedo,
A. Contu,
N. Cooke,
I. Corredoira ,
A. Correia,
G. Corti,
J.J. Cottee Meldrum,
B. Couturier,
D.C. Craik,
M. Cruz Torres,
E. Curras Rivera,
R. Currie,
C.L. Da Silva,
S. Dadabaev,
L. Dai,
X. Dai,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
J. Daniel,
A. Danilina,
P. d'Argent,
A.  Davidson,
J.E. Davies,
A. Davis,
O. De Aguiar Francisco,
C. De Angelis,
F. De Benedetti,
J. de Boer,
K. De Bruyn,
S. De Capua,
M. De Cian,
U. De Freitas Carneiro Da Graca,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
F. De Vellis,
J.A. de Vries,
F. Debernardis,
D. Decamp,
V. Dedu,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
J. Deng,
V. Denysenko,
O. Deschamps,
F. Dettori,
B. Dey,
P. Di Nezza,
I. Diachkov,
S. Didenko,
S. Ding,
L. Dittmann,
V. Dobishuk,
A. D.  Docheva,
C. Dong,
A.M. Donohoe,
F. Dordei,
A.C. dos Reis,
A. D.  Dowling,
W. Duan,
P. Duda,
M.W. Dudek,
L. Dufour,
V. Duk,
P. Durante,
M. M. Duras,
J.M. Durham,
O. D.  Durmus,
A. Dziurda,
A. Dzyuba,
S. Easo,
E. Eckstein,
U. Egede,
A. Egorychev,
V. Egorychev,
S. Eisenhardt,
E. Ejopu,
S. Ek-In,
L. Eklund,
M. Elashri,
J. Ellbracht,
S. Ely,
A. Ene,
E. Epple,
J. Eschle,
S. Esen,
T. Evans,
F. Fabiano,
L.N. Falcao,
Y. Fan,
B. Fang,
L. Fantini,
M. Faria,
K.   Farmer,
D. Fazzini,
L. Felkowski,
M. Feng,
M. Feo,
M. Fernandez Gomez,
A.D. Fernez,
F. Ferrari,
F. Ferreira Rodrigues,
S. Ferreres Sole,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
K.M. Fischer,
D.S. Fitzgerald,
C. Fitzpatrick,
F. Fleuret,
M. Fontana,
L. F.  Foreman,
R. Forty,
D. Foulds-Holt,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. Fuehring,
Y. Fujii,
T. Fulghesu,
E. Gabriel,
G. Galati,
M.D. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
M. Gandelman,
P. Gandini,
B.  Ganie,
H. Gao,
R. Gao,
Y. Gao,
Y. Gao,
Y. Gao,
M. Garau,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
K. G.  Garg,
L. Garrido,
C. Gaspar,
R.E. Geertsema,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
Z. Ghorbanimoghaddam,
L. Giambastiani,
F. I. Giasemis,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent{\`u},
P. Gironella Gironell,
C. Giugliano,
M.A. Giza,
E.L. Gkougkousis,
F.C. Glaser,
V.V. Gligorov,
C. G{\"o}bel,
E. Golobardes,
D. Golubkov,
A. Golutvin,
A. Gomes,
S. Gomez Fernandez,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
J. A. Gooding,
I.V. Gorelov,
C. Gotti,
J.P. Grabowski,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
L. Grazette,
G. Graziani,
A. T. Grecu,
L.M. Greeven,
N.A. Grieser,
L. Grillo,
S. Gromov,
C.  Gu,
M. Guarise,
M. Guittiere,
V. Guliaeva,
P. A. G{\"u}nther,
A.-K. Guseinov,
E. Gushchin,
Y. Guz,
T. Gys,
K. Habermann,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
J. Haimberger,
M. Hajheidari,
M.M. Halvorsen,
P.M. Hamilton,
J. Hammerich,
Q. Han,
X. Han,
S. Hansmann-Menzemer,
L. Hao,
N. Harnew,
M. Hartmann,
J. He,
F. Hemmer,
C. Henderson,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Herd,
P. Herrero Gascon,
J. Heuel,
A. Hicheur,
G. Hijano Mendizabal,
D. Hill,
S.E. Hollitt,
J. Horswill,
R. Hou,
Y. Hou,
N. Howarth,
J. Hu,
J. Hu,
W. Hu,
X. Hu,
W. Huang,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
D. Ilin,
P. Ilten,
A. Inglessi,
A. Iniukhin,
A. Ishteev,
K. Ivshin,
R. Jacobsson,
H. Jage,
S.J. Jaimes Elles,
S. Jakobsen,
E. Jans,
B.K. Jashal,
A. Jawahery,
V. Jevtic,
E. Jiang,
X. Jiang,
Y. Jiang,
Y. J.  Jiang,
M. John,
D. Johnson,
C.R. Jones,
T.P. Jones,
S. Joshi,
B. Jost,
N. Jurik,
I. Juszczak,
D. Kaminaris,
S. Kandybei,
Y. Kang,
C. Kar,
M. Karacson,
D. Karpenkov,
A. Kauniskangas,
J.W. Kautz,
F. Keizer,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
G. Khreich,
T. Kirn,
V.S. Kirsebom,
O. Kitouni,
S. Klaver,
N. Kleijne,
K. Klimaszewski,
M.R. Kmiec,
S. Koliiev,
L. Kolk,
A. Konoplyannikov,
P. Kopciewicz,
P. Koppenburg,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
A. Kozachuk,
P. Kravchenko,
L. Kravchuk,
M. Kreps,
P. Krokovny,
W. Krupa,
W. Krzemien,
O.K. Kshyvanskyi,
J. Kubat,
S. Kubis,
M. Kucharczyk,
V. Kudryavtsev,
E. Kulikova,
A. Kupsc,
B. K.  Kutsenko,
D. Lacarrere,
A. Lai,
A. Lampis,
D. Lancierini,
C. Landesa Gomez,
J.J. Lane,
R. Lane,
C. Langenbruch,
J. Langer,
O. Lantwin,
T. Latham,
F. Lazzari,
C. Lazzeroni,
R. Le Gac,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
M. Lehuraux,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
B. Leverington,
A. Li,
H. Li,
K. Li,
L. Li,
P. Li,
P.-R. Li,
Q.  Li,
S. Li,
T. Li,
T. Li,
Y. Li,
Y. Li,
Z. Lian,
X. Liang,
S. Libralon,
C. Lin,
T. Lin,
R. Lindner,
V. Lisovskyi,
R. Litvinov,
F. L.  Liu,
G. Liu,
K. Liu,
S. Liu,
Y. Liu,
Y. Liu,
Y. L.  Liu,
A. Lobo Salvia,
A. Loi,
J. Lomba Castro,
T. Long,
J.H. Lopes,
A. Lopez Huertas,
S. L{\'o}pez Soli{\~n}o,
C. Lucarelli,
D. Lucchesi,
M. Lucio Martinez,
V. Lukashenko,
Y. Luo,
A. Lupato,
E. Luppi,
K. Lynch,
X.-R. Lyu,
G. M.  Ma,
R. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
B. M.  Mack,
I. Mackay,
L. M.  Mackey,
L.R. Madhan Mohan,
M. J.  Madurai,
A. Maevskiy,
D. Magdalinski,
D. Maisuzenko,
M.W. Majewski,
J.J. Malczewski,
S. Malde,
L. Malentacca,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
C. Mancuso,
R. Manera Escalero,
D. Manuzzi,
D. Marangotto,
J.F. Marchand,
R. Marchevski,
U. Marconi,
S. Mariani,
C. Marin Benito,
J. Marks,
A.M. Marshall,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
R. Matev,
A. Mathad,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
P. Mayencourt,
M. Mazurek,
M. McCann,
L. Mcconnell,
T.H. McGrath,
N.T. McHugh,
A. McNab,
R. McNulty,
B. Meadows,
G. Meier,
D. Melnychuk,
F. M.  Meng,
M. Merk,
A. Merli,
L. Meyer Garcia,
D. Miao,
H. Miao,
M. Mikhasenko,
D.A. Milanes,
A. Minotti,
E. Minucci,
T. Miralles,
B. Mitreska,
D.S. Mitzel,
A. Modak,
A. M{\"o}dden ,
R.A. Mohammed,
R.D. Moise,
S. Mokhnenko,
T. Momb{\"a}cher,
M. Monk,
S. Monteil,
A. Morcillo Gomez,
G. Morello,
M.J. Morello,
M.P. Morgenthaler,
A.B. Morris,
A.G. Morris,
R. Mountain,
H. Mu,
Z. M.  Mu,
E. Muhammad,
F. Muheim,
M. Mulder,
K. M{\"u}ller,
F. Mu{\~n}oz-Rojas,
R. Murta,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
P. Neustroev,
J. Nicolini,
D. Nicotra,
E.M. Niel,
N. Nikitin,
P. Nogga,
N.S. Nolte,
C. Normand,
J. Novoa Fernandez,
G. Nowak,
C. Nunez,
H. N.  Nur,
A. Oblakowska-Mucha,
V. Obraztsov,
T. Oeser,
S. Okamura,
A. Okhotnikov,
O. Okhrimenko,
R. Oldeman,
F. Oliva,
M. Olocco,
C.J.G. Onderwater,
R.H. O'Neil,
J.M. Otalora Goicochea,
P. Owen,
A. Oyanguren,
O. Ozcelik,
K.O. Padeken,
B. Pagare,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
G. Panshin,
L. Paolucci,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
C. Parkes,
B. Passalacqua,
G. Passaleva,
D. Passaro,
A. Pastore,
M. Patel,
J. Patoc,
C. Patrignani,
C.J. Pawley,
A. Pellegrino,
J.  Peng,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
A. Pereiro Castro,
P. Perret,
A. Perro,
K. Petridis,
A. Petrolini,
J. P.  Pfaller,
H. Pham,
L. Pica,
M. Piccini,
B. Pietrzyk,
G. Pietrzyk,
D. Pinci,
F. Pisani,
M. Pizzichemi,
V. Placinta,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
S. Poslavskii,
K. Prasanth,
C. Prouve,
V. Pugatch,
G. Punzi,
W. Qian,
N. Qin,
S. Qu,
R. Quagliani,
R.I. Rabadan Trejo,
J.H. Rademacker,
M. Rama,
M.  Ram\'{i}rez Garc\'{i}a,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Rebollo De Miguel,
F. Redi,
J. Reich,
F. Reiss,
Z. Ren,
P.K. Resmi,
R. Ribatti,
G. R.  Ricart,
D. Riccardi,
S. Ricciardi,
K. Richardson,
M. Richardson-Slipper,
K. Rinnert,
P. Robbe,
G. Robertson,
E. Rodrigues,
E. Rodriguez Fernandez,
J.A. Rodriguez Lopez,
E. Rodriguez Rodriguez,
A. Rogovskiy,
D.L. Rolf,
P. Roloff,
V. Romanovskiy,
M. Romero Lamas,
A. Romero Vidal,
G. Romolini,
F. Ronchetti,
M. Rotondo,
S. R.  Roy,
M.S. Rudolph,
T. Ruf,
M. Ruiz Diaz,
R.A. Ruiz Fernandez,
J. Ruiz Vidal,
A. Ryzhikov,
J. Ryzka,
J. J. Saavedra-Arias,
J.J. Saborido Silva,
R. Sadek,
N. Sagidova,
D. Sahoo,
N. Sahoo,
B. Saitta,
M. Salomoni,
C. Sanchez Gras,
I. Sanderswood,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
L. Santoro ,
E. Santovetti,
A. Saputi,
D. Saranin,
G. Sarpis,
M. Sarpis,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
L.G. Scantlebury Smead,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
S. Schmitt,
H. Schmitz,
O. Schneider,
A. Schopper,
N. Schulte,
S. Schulte,
M.H. Schune,
R. Schwemmer,
G. Schwering,
B. Sciascia,
A. Sciuccati,
S. Sellam,
A. Semennikov,
T. Senger,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
A. Seuthe,
Y. Shang,
D.M. Shangase,
M. Shapkin,
R. S.  Sharma,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
S. Sheng,
V. Shevchenko,
B. Shi,
Q. Shi,
E.B. Shields,
Y. Shimizu,
E. Shmanin,
R. Shorkin,
J.D. Shupperd,
R. Silva Coutinho,
G. Simi,
S. Simone,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
J.C. Smallwood,
E. Smith,
K. Smith,
M. Smith,
A. Snoch,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solomin,
A. Solovev,
I. Solovyev,
R. Song,
Y. Song,
Y. Song,
Y. S.  Song,
F.L. Souza De Almeida,
B. Souza De Paula,
E. Spadaro Norella,
E. Spedicato,
J.G. Speer,
E. Spiridenkov,
P. Spradlin,
V. Sriskaran,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
E.N. Stein,
O. Steinkamp,
O. Stenyakin,
H. Stevens,
D. Strekalina,
Y. Su,
F. Suljik,
J. Sun,
L. Sun,
Y. Sun,
D. S.  Sundfeld Lima,
W. Sutcliffe,
P.N. Swallow,
F. Swystun,
A. Szabelski,
T. Szumlak,
Y. Tan,
M.D. Tat,
A. Terentev,
F. Terzuoli,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
L. Tomassetti,
G. Tonani,
X. Tong,
D. Torres Machado,
L. Toscano,
D.Y. Tou,
C. Trippl,
G. Tuci,
N. Tuning,
L.H. Uecker,
A. Ukleja,
D.J. Unverzagt,
E. Ursov,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
V. Vagnoni,
A. Valassi,
G. Valenti,
N. Valls Canudas,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
R. Van Laak,
M. van Veghel,
G. Vasquez,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Vesterinen,
M. Vieites Diaz,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
F.C. Volle,
D. vom Bruch,
N. Voropaev,
K. Vos,
G. Vouters,
C. Vrahas,
J. Wagner,
J. Walsh,
E.J. Walton,
G. Wan,
C. Wang,
G. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
N. W.  Wang,
R. Wang,
X. Wang,
X. Wang,
X. W.  Wang,
Z. Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
M. Waterlaat,
N.K. Watson,
D. Websdale,
Y. Wei,
J. Wendel,
B.D.C. Westhenry,
D.J. White,
M. Whitehead,
A.R. Wiederhold,
D. Wiedner,
G. Wilkinson,
M.K. Wilkinson,
M. Williams,
M.R.J. Williams,
R. Williams,
F.F. Wilson,
W. Wislicki,
M. Witek,
L. Witola,
C.P. Wong,
G. Wormser,
S.A. Wotton,
H. Wu,
J. Wu,
Y. Wu,
K. Wyllie,
S. Xian,
Z. Xiang,
Y. Xie,
A. Xu,
J. Xu,
L. Xu,
L. Xu,
M. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
D. Yang,
S. Yang,
X. Yang,
Y. Yang,
Z. Yang,
Z. Yang,
V. Yeroshenko,
H. Yeung,
H. Yin,
C. Y.  Yu,
J. Yu,
X. Yuan,
E. Zaffaroni,
M. Zavertyaev,
M. Zdybal,
M. Zeng,
C. Zhang,
D. Zhang,
J. Zhang,
L. Zhang,
S. Zhang,
S. Zhang,
Y. Zhang,
Y. Z.  Zhang,
Y. Zhao,
A. Zharkova,
A. Zhelezov,
X. Z.  Zheng,
Y. Zheng,
T. Zhou,
X. Zhou,
Y. Zhou,
V. Zhovkovska,
L. Z.  Zhu,
X. Zhu,
X. Zhu,
V. Zhukov,
J. Zhuo,
Q. Zou,
D. Zuliani,
G. Zunica

==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright && dvips -z -o upright.ps upright && ps2pdf upright.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib) $(wildcard *.bst)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prl.pdf

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 

# Make the upright version
upright: 
	$(BUILDCOMMANDUPRIGHT)



==> tables/Dresonances.tex <==
\begin{tabular}{c|clc}
	Resonance & $J^{P}$ & Mass [MeV] & Width [MeV]\\
	\midrule
	$D_{1}(2420)$ &$1^{+}$ & $2\,422.1\pm0.6$ & $31.3\pm1.9$\\
	$D_{1}(2430)$ &$1^{+}$ & $2\,412\phantom{.0}\pm9\phantom{.0}$ & $314\pm29$\\
        $D_{2}^{*}(2460)$ & $2^{+}$ & $2\,461.1\;{}^{+0.7}_{-0.8}$ & $47.3\pm0.8$\\
	\midrule
	$D_{0}(2550)$ &$0^{-}$ & $2\,549\phantom{.0}\pm19\phantom{.}$ & $165\pm24$\\
	$D_{1}^{*}(2600)$ &$1^{-}$ & $2\,627\phantom{.0}\pm10\phantom{.}$ & $141\pm23$\\
	$D_{2}(2740)$ &$2^{-}$ & $2\,747\phantom{.0}\pm6\phantom{.0}$ & $\phantom{0}88\pm19$\\
	$D_{3}^{*}(2750)$ &$3^{-}$ & $2\,763.1\pm 3.2$ & $66\pm 5$\\
\end{tabular}

==> tables/br_rel_syst_unc_table.tex <==
\begin{tabular}{l|cc}
Source of systematic uncertainty & $\delta\mathcal{R}$ [\%] & $\delta\mathcal{R}^{*}$ [\%] \\
\midrule
Fully reconstructed signal model & 3.5 & 8.4 \\
Combinatorial background model & 3.7 & 2.8 \\
Partially reconstructed signal model & 1.0 & 2.9 \\
Non-$D_s$ fraction estimation & 0.1 & 0.2 \\
Efficiency, PID correction & 0.6 & 1.2 \\
Efficiency, sample size & 0.6 & 0.5 \\
Efficiency, trigger correction & 1.2 & 0.3 \\
Efficiency non-uniformity correction & 2.3 & 4.8 \\
\end{tabular}


==> tables/fractions.tex <==
\begin{tabular}{l|rr}
Component & Fit fraction [\%] & Phase [rad] \\
\midrule
$D_1(2420)$ S-wave  &  $3.8\pm 1.7\pm 0.8^{+1.3}_{-0.1}$ & $-1.96\pm 0.16\pm 0.10^{+0.17}_{-0.05}$ \\
$D_1(2420)$ D-wave  & $71.0\pm 4.4\pm 4.6^{+0.0}_{-6.0}$ & 0 (fixed) \\
$D_1(2430)$ S-wave  & $14.2\pm 2.5\pm 2.4^{+3.1}_{-2.0}$ & $+0.14\pm 0.11\pm 0.13^{+0.06}_{-0.18}$ \\
$D_1(2430)$ D-wave  &  $0.5\pm 0.9\pm 1.5^{+0.2}_{-0.5}$ & $-2.99\pm 0.42\pm 0.84^{+0.23}_{-0.55}$ \\
$D^*_2(2460)$         & $11.7\pm 1.4\pm 0.8^{+0.0}_{-0.7}$ & $+3.14\pm 0.11\pm 0.14^{+0.05}_{-0.04}$ \\
$D_0(2550)$           &  $2.3\pm 0.8\pm 0.7^{+0.3}_{-1.7}$ & $-2.24\pm 0.21\pm 0.26^{+0.05}_{-0.25}$ \\
$D^*_1(2600)$         &  $4.8\pm 1.0\pm 0.9^{+1.1}_{-2.0}$ & $+0.32\pm 0.16\pm 0.16^{+0.37}_{-0.01}$ \\
$D_2(2740)$ P-wave  &  $0.4\pm 0.4\pm 0.2^{+0.1}_{-0.1}$ & $-0.02\pm 0.56\pm 0.32^{+0.16}_{-0.59}$ \\
$D_2(2740)$ F-wave  &  $2.3\pm 0.7\pm 0.9^{+0.4}_{-0.1}$ & $-0.09\pm 0.27\pm 0.21^{+0.08}_{-0.23}$ \\
\midrule
Sum of fit fractions  &  $111.0\pm 5.2\pm 4.2\phantom{{}^{+0.0}}$ & \\
\end{tabular}



==> tables/results.tex <==
\begin{tabular}{ll|ccccc} 
          &            &           & Floated      &      & NR                & NR, \\ 
Component & Parameter  & Baseline  & $D_1(2430)$  & QMI  & $D^*\pi$ $1^{-}$  & \tcsbar \\ \midrule
  & $-\ln\mathcal{L}$ & $-1670.16$ & $-1671.12$ & $-1674.18$ & $-1683.01$ & $-1694.94$ \\ 
\midrule 
  $D_1(2420)$ & ${\rm Re}(c_{0,1})$& $-0.088 \pm 0.033$ & $-0.08 \pm 0.05$ & $-0.06 \pm 0.04$ & $-0.085 \pm 0.034$ & $-0.101 \pm 0.035$ \\ 
 & ${\rm Im}(c_{0,1})$& $-0.22 \pm 0.06$ & $-0.26 \pm 0.06$ & $-0.26 \pm 0.05$ & $-0.22 \pm 0.05$ & $-0.22 \pm 0.06$ \\ 
 & ${\rm Re}(c_{2,1})$& $\phantom{-}1.0$ (fixed) & $\phantom{-}1.0$ (fixed) & $\phantom{-}1.0$ (fixed) & $\phantom{-}1.0$ (fixed) & $\phantom{-}1.0$ (fixed) \\ 
 & ${\rm Im}(c_{2,1})$& $\phantom{-}0.0$ (fixed) & $\phantom{-}0.0$ (fixed) & $\phantom{-}0.0$ (fixed) & $\phantom{-}0.0$ (fixed) & $\phantom{-}0.0$ (fixed) \\ 
 & $\mathcal{F}$(S-wave) & $\phantom{-}0.038 \pm 0.017$ & $\phantom{-}0.050 \pm 0.024$ & $\phantom{-}0.046 \pm 0.018$ & $\phantom{-}0.040 \pm 0.018$ & $\phantom{-}0.036 \pm 0.019$ \\ 
 & $\mathcal{F}$(D-wave) & $\phantom{-}0.71 \pm 0.04$ & $\phantom{-}0.71 \pm 0.05$ & $\phantom{-}0.651 \pm 0.022$ & $\phantom{-}0.71 \pm 0.04$ & $\phantom{-}0.66 \pm 0.04$ \\ 
\midrule 
  $D_1(2430)$ & ${\rm Re}(c_{0,1})$& $\phantom{-}1.64 \pm 0.16$ & $\phantom{-}1.44 \pm 0.25$  & - & $\phantom{-}1.60 \pm 0.16$ & $\phantom{-}1.90 \pm 0.20$ \\ 
 & ${\rm Im}(c_{0,1})$& $\phantom{-}0.23 \pm 0.17$ & $-0.06 \pm 0.24$  & - & $\phantom{-}0.32 \pm 0.17$ & $\phantom{-}0.05 \pm 0.24$ \\ 
 & ${\rm Re}(c_{2,1})$& $-0.33 \pm 0.26$ & $-0.35 \pm 0.23$  & - & $-0.36 \pm 0.28$ & $-0.11 \pm 0.26$ \\ 
 & ${\rm Im}(c_{2,1})$& $-0.05 \pm 0.13$ & $\phantom{-}0.03 \pm 0.15$  & - & $-0.02 \pm 0.13$ & $-0.09 \pm 0.14$ \\ 
 & $m_0$ [$\gev\,$]& $2.412$ (fixed) & $\phantom{-}2.378 \pm 0.025$  & - & $2.412$ (fixed) & $2.412$ (fixed) \\ 
 & $\Gamma_0$ [$\gev\,$]& $0.314$ (fixed) & $\phantom{-}0.24 \pm 0.06$  & - & $0.314$ (fixed) & $0.314$ (fixed) \\ 
 & $\mathcal{F}$(S-wave) & $\phantom{-}0.142 \pm 0.025$ & $\phantom{-}0.139 \pm 0.031$  & - & $\phantom{-}0.137 \pm 0.025$ & $\phantom{-}0.17 \pm 0.04$ \\ 
 & $\mathcal{F}$(D-wave) & $\phantom{-}0.005 \pm 0.009$ & $\phantom{-}0.007 \pm 0.012$  & - & $\phantom{-}0.006 \pm 0.008$ & $\phantom{-}0.001 \pm 0.004$ \\ 
\midrule 
  $1^+S$ QMI  & $\mathcal{F}$(S-wave)  & -  & - & $\phantom{-}0.122 \pm 0.024$  & -  & - \\ 
\midrule
  $D_2^*(2460)$ & ${\rm Re}(c_{2,1})$& $-0.64 \pm 0.04$ & $-0.64 \pm 0.05$ & $-0.67 \pm 0.04$ & $-0.62 \pm 0.05$ & $-0.66 \pm 0.05$ \\ 
 & ${\rm Im}(c_{2,1})$& $\phantom{-}0.00 \pm 0.07$ & $-0.00 \pm 0.07$ & $\phantom{-}0.03 \pm 0.07$ & $\phantom{-}0.01 \pm 0.07$ & $-0.03 \pm 0.07$ \\ 
 & $\mathcal{F}$(D-wave) & $\phantom{-}0.117 \pm 0.014$ & $\phantom{-}0.116 \pm 0.014$ & $\phantom{-}0.116 \pm 0.014$ & $\phantom{-}0.109 \pm 0.014$ & $\phantom{-}0.115 \pm 0.016$ \\ 
\midrule 
  $D_0(2550)$ & ${\rm Re}(c_{1,1})$& $-0.15 \pm 0.05$ & $-0.15 \pm 0.05$ & $-0.21 \pm 0.06$ & $-0.15 \pm 0.06$ & $-0.11 \pm 0.06$ \\ 
 & ${\rm Im}(c_{1,1})$& $-0.19 \pm 0.05$ & $-0.19 \pm 0.05$ & $-0.18 \pm 0.05$ & $-0.21 \pm 0.06$ & $-0.08 \pm 0.06$ \\ 
 & $\mathcal{F}$(P-wave) & $\phantom{-}0.023 \pm 0.008$ & $\phantom{-}0.023 \pm 0.008$ & $\phantom{-}0.026 \pm 0.008$ & $\phantom{-}0.027 \pm 0.009$ & $\phantom{-}0.007 \pm 0.005$ \\ 
\midrule 
  $D_1^*(2600)$ & ${\rm Re}(c_{1,1})$& $\phantom{-}0.53 \pm 0.07$ & $\phantom{-}0.54 \pm 0.07$ & $\phantom{-}0.54 \pm 0.07$ & $\phantom{-}0.34 \pm 0.09$ & $\phantom{-}0.50 \pm 0.09$ \\ 
 & ${\rm Im}(c_{1,1})$& $\phantom{-}0.17 \pm 0.09$ & $\phantom{-}0.17 \pm 0.09$ & $\phantom{-}0.19 \pm 0.10$ & $\phantom{-}0.25 \pm 0.12$ & $\phantom{-}0.41 \pm 0.11$ \\ 
 & $\mathcal{F}$(P-wave) & $\phantom{-}0.048 \pm 0.010$ & $\phantom{-}0.049 \pm 0.010$ & $\phantom{-}0.047 \pm 0.009$ & $\phantom{-}0.028 \pm 0.013$ & $\phantom{-}0.059 \pm 0.015$ \\ 
\midrule 
  $D_2(2740)$ & ${\rm Re}(c_{1,1})$& $\phantom{-}0.15 \pm 0.07$ & $\phantom{-}0.17 \pm 0.06$ & $\phantom{-}0.19 \pm 0.07$ & $\phantom{-}0.16 \pm 0.07$ & $\phantom{-}0.11 \pm 0.07$ \\ 
 & ${\rm Im}(c_{1,1})$& $-0.00 \pm 0.09$ & $\phantom{-}0.00 \pm 0.09$ & $\phantom{-}0.03 \pm 0.08$ & $\phantom{-}0.00 \pm 0.09$ & $-0.08 \pm 0.11$ \\ 
 & ${\rm Re}(c_{3,1})$& $\phantom{-}0.39 \pm 0.07$ & $\phantom{-}0.40 \pm 0.07$ & $\phantom{-}0.40 \pm 0.08$ & $\phantom{-}0.39 \pm 0.08$ & $\phantom{-}0.42 \pm 0.07$ \\ 
 & ${\rm Im}(c_{3,1})$& $-0.04 \pm 0.11$ & $-0.03 \pm 0.11$ & $-0.05 \pm 0.10$ & $-0.00 \pm 0.12$ & $-0.14 \pm 0.11$ \\ 
 & $\mathcal{F}$(P-wave) & $\phantom{-}0.004 \pm 0.004$ & $\phantom{-}0.004 \pm 0.004$ & $\phantom{-}0.005 \pm 0.005$ & $\phantom{-}0.004 \pm 0.004$ & $\phantom{-}0.003 \pm 0.004$ \\ 
 & $\mathcal{F}$(F-wave) & $\phantom{-}0.023 \pm 0.007$ & $\phantom{-}0.025 \pm 0.008$ & $\phantom{-}0.023 \pm 0.007$ & $\phantom{-}0.022 \pm 0.008$ & $\phantom{-}0.027 \pm 0.008$ \\ 
\midrule 
  NR $1^-$ & ${\rm Re}(c_{1,1})$ & -  & -  & - & $\phantom{-}0.053 \pm 0.018$  & - \\ 
 & ${\rm Im}(c_{1,1})$ & -  & -  & - & $\phantom{-}0.034 \pm 0.020$  & - \\ 
 & $\alpha$ [$\gev^{-2}\,$] & -  & -  & - & $\phantom{-}0.99 \pm 0.30$  & - \\ 
 & $\mathcal{F}$(P-wave)  & -  & -  & - & $\phantom{-}0.025 \pm 0.009$  & - \\ 
\midrule 
  NR $\Dsp\pip$ & ${\rm Re}(c_{0,0})$ & -  & -  & -  & - & $-0.006 \pm 0.008$ \\ 
 & ${\rm Im}(c_{0,0})$ & -  & -  & -  & - & $\phantom{-}0.021 \pm 0.014$ \\ 
 & ${\rm Re}(c_{1,1})$ & -  & -  & -  & - & $\phantom{-}0.063 \pm 0.035$ \\ 
 & ${\rm Im}(c_{1,1})$ & -  & -  & -  & - & $\phantom{-}0.007 \pm 0.013$ \\ 
 & ${\rm Re}(c_{2,2})$ & -  & -  & -  & - & $-0.062 \pm 0.033$ \\ 
 & ${\rm Im}(c_{2,2})$ & -  & -  & -  & - & $\phantom{-}0.034 \pm 0.026$ \\ 
 & $\alpha$  [$\gev^{-2}\,$] & -  & -  & -  & - & $-0.32 \pm 0.14$ \\ 
 & $\mathcal{F}$(S-wave)  & -  & -  & -  & - & $\phantom{-}0.028 \pm 0.014$ \\ 
 & $\mathcal{F}$(P-wave)  & -  & -  & -  & - & $\phantom{-}0.048 \pm 0.014$ \\ 
 & $\mathcal{F}$(D-wave)  & -  & -  & -  & - & $\phantom{-}0.019 \pm 0.010$ \\ 
\midrule 
  \tcsbar & ${\rm Re}(c_{1,1})$ & -  & -  & -  & - & $\phantom{-}0.17 \pm 0.05$ \\ 
 & ${\rm Im}(c_{1,1})$ & -  & -  & -  & - & $\phantom{-}0.04 \pm 0.07$ \\ 
 & $\mathcal{F}$(P-wave)  & -  & -  & -  & - & $\phantom{-}0.012 \pm 0.008$ \\ 
\end{tabular} 


==> tables/results_spline.tex <==
\begin{tabular}{l|cc} 
Parameter  & ${\rm Re}(f_i)$  & ${\rm Im}(f_i)$  \\ \midrule
 $f_0$ & $\phantom{-}0.2 \pm 2.8$   & $\phantom{-}0.7 \pm 2.4$ \\ 
 $f_1$ & $\phantom{-}0.9 \pm 1.2$   & $\phantom{-}1.7 \pm 0.9$ \\ 
 $f_2$ & $\phantom{-}0.7 \pm 0.6$   & $\phantom{-}2.5 \pm 0.4$ \\ 
 $f_3$ &          $-0.72 \pm 0.19$  & $\phantom{-}1.12 \pm 0.26$ \\ 
 $f_4$ & $\phantom{-}0.02 \pm 0.17$ & $\phantom{-}0.31 \pm 0.22$ \\ 
 $f_5$ & $-1.4 \pm 0.5$             & $-0.4 \pm 0.9$ \\ 
\end{tabular} 



==> tables/unc1.tex <==
\begin{tabular}{l|rrrrrrrrrrrr}
{} &  \begin{sideways}Accept., sample size\end{sideways} &  \begin{sideways}Accept., ANN param.\end{sideways} &  \begin{sideways}Efficiency, sample size\end{sideways} &  \begin{sideways}Efficiency, ANN param.\end{sideways} &  \begin{sideways}Efficiency, PID corr.\end{sideways} &  \begin{sideways}Efficiency, L0 corr.\end{sideways} &  \begin{sideways}Comb. bkg., sample size\end{sideways} &  \begin{sideways}Comb. bkg., ANN param.\end{sideways} &  \begin{sideways}Comb. bkg. fraction\end{sideways} &  \begin{sideways}Non-$D_s$ bkg., sample size\end{sideways} &  \begin{sideways}Non-$D_s$ bkg., ANN param.\end{sideways} &  \begin{sideways}Non-$D_s$ bkg. fraction\end{sideways} \\
\midrule
$D_1(2420)$ ${\rm Re}(c_{0,1})$       &                                              0.002 &                                              0.004 &                                              0.008 &                                              0.008 &                                              0.001 &                                              0.002 &                                              0.003 &                                              0.005 &                                              0.002 &                                              0.001 &                                              0.005 &                                              0.003 \\
$D_1(2420)$ ${\rm Im}(c_{0,1})$       &                                              0.003 &                                              0.004 &                                              0.006 &                                              0.007 &                                              0.005 &                                              0.002 &                                              0.005 &                                              0.011 &                                              0.003 &                                              0.002 &                                              0.010 &                                              0.002 \\
$D_1(2430)$ ${\rm Re}(c_{0,1})$       &                                              0.008 &                                              0.005 &                                              0.017 &                                              0.019 &                                              0.028 &                                              0.009 &                                              0.030 &                                              0.050 &                                              0.017 &                                              0.011 &                                              0.022 &                                              0.021 \\
$D_1(2430)$ ${\rm Im}(c_{0,1})$       &                                              0.005 &                                              0.003 &                                              0.012 &                                              0.013 &                                              0.005 &                                              0.007 &                                              0.014 &                                              0.069 &                                              0.010 &                                              0.008 &                                              0.002 &                                              0.008 \\
$D_1(2430)$ ${\rm Re}(c_{2,1})$       &                                              0.009 &                                              0.012 &                                              0.015 &                                              0.010 &                                              0.023 &                                              0.000 &                                              0.031 &                                              0.032 &                                              0.007 &                                              0.023 &                                              0.038 &                                              0.012 \\
$D_1(2430)$ ${\rm Im}(c_{2,1})$       &                                              0.005 &                                              0.004 &                                              0.009 &                                              0.008 &                                              0.003 &                                              0.001 &                                              0.014 &                                              0.014 &                                              0.001 &                                              0.008 &                                              0.019 &                                              0.001 \\
$D_2^*(2460)$ ${\rm Re}(c_{2,1})$     &                                              0.003 &                                              0.004 &                                              0.004 &                                              0.004 &                                              0.005 &                                              0.006 &                                              0.003 &                                              0.002 &                                              0.001 &                                              0.002 &                                              0.006 &                                              0.001 \\
$D_2^*(2460)$ ${\rm Im}(c_{2,1})$     &                                              0.003 &                                              0.006 &                                              0.009 &                                              0.007 &                                              0.003 &                                              0.001 &                                              0.005 &                                              0.006 &                                              0.001 &                                              0.002 &                                              0.005 &                                              0.002 \\
$D_0(2550)$ ${\rm Re}(c_{1,1})$       &                                              0.002 &                                              0.002 &                                              0.005 &                                              0.007 &                                              0.006 &                                              0.006 &                                              0.006 &                                              0.011 &                                              0.001 &                                              0.005 &                                              0.003 &                                              0.001 \\
$D_0(2550)$ ${\rm Im}(c_{1,1})$       &                                              0.004 &                                              0.003 &                                              0.008 &                                              0.010 &                                              0.004 &                                              0.001 &                                              0.006 &                                              0.014 &                                              0.001 &                                              0.005 &                                              0.005 &                                              0.001 \\
$D_1^*(2600)$ ${\rm Re}(c_{1,1})$     &                                              0.003 &                                              0.005 &                                              0.005 &                                              0.003 &                                              0.003 &                                              0.008 &                                              0.006 &                                              0.009 &                                              0.002 &                                              0.006 &                                              0.004 &                                              0.007 \\
$D_1^*(2600)$ ${\rm Im}(c_{1,1})$     &                                              0.004 &                                              0.002 &                                              0.008 &                                              0.011 &                                              0.010 &                                              0.007 &                                              0.008 &                                              0.019 &                                              0.001 &                                              0.006 &                                              0.007 &                                              0.003 \\
$D_2(2740)$ ${\rm Re}(c_{1,1})$       &                                              0.001 &                                              0.001 &                                              0.005 &                                              0.004 &                                              0.003 &                                              0.001 &                                              0.005 &                                              0.003 &                                              0.001 &                                              0.004 &                                              0.003 &                                              0.002 \\
$D_2(2740)$ ${\rm Im}(c_{1,1})$       &                                              0.002 &                                              0.001 &                                              0.006 &                                              0.005 &                                              0.004 &                                              0.006 &                                              0.011 &                                              0.016 &                                              0.002 &                                              0.003 &                                              0.009 &                                              0.003 \\
$D_2(2740)$ ${\rm Re}(c_{3,1})$       &                                              0.001 &                                              0.002 &                                              0.007 &                                              0.005 &                                              0.007 &                                              0.000 &                                              0.009 &                                              0.024 &                                              0.002 &                                              0.007 &                                              0.031 &                                              0.004 \\
$D_2(2740)$ ${\rm Im}(c_{3,1})$       &                                              0.004 &                                              0.003 &                                              0.009 &                                              0.006 &                                              0.007 &                                              0.005 &                                              0.010 &                                              0.020 &                                              0.001 &                                              0.011 &                                              0.008 &                                              0.002 \\
\midrule
$\mathcal{F}$($D_1(2420)$ S-wave)          &                                              0.001 &                                              0.001 &                                              0.002 &                                              0.002 &                                              0.001 &                                              0.000 &                                              0.001 &                                              0.003 &                                              0.001 &                                              0.001 &                                              0.003 &                                              0.001 \\
$\mathcal{F}$($D_1(2420)$ D-wave)          &                                              0.002 &                                              0.005 &                                              0.005 &                                              0.003 &                                              0.003 &                                              0.004 &                                              0.004 &                                              0.004 &                                              0.001 &                                              0.004 &                                              0.007 &                                              0.005 \\
$\mathcal{F}$($D_1(2430)$ S-wave)          &                                              0.001 &                                              0.001 &                                              0.003 &                                              0.003 &                                              0.004 &                                              0.001 &                                              0.005 &                                              0.007 &                                              0.002 &                                              0.001 &                                              0.002 &                                              0.002 \\
$\mathcal{F}$($D_1(2430)$ D-wave)          &                                              0.000 &                                              0.000 &                                              0.000 &                                              0.000 &                                              0.001 &                                              0.000 &                                              0.001 &                                              0.001 &                                              0.000 &                                              0.001 &                                              0.001 &                                              0.000 \\
$\mathcal{F}$($D_2(2460)$ D-wave)                 &                                              0.001 &                                              0.001 &                                              0.001 &                                              0.002 &                                              0.001 &                                              0.002 &                                              0.001 &                                              0.000 &                                              0.000 &                                              0.001 &                                              0.001 &                                              0.000 \\
$\mathcal{F}$($D_0(2550)$ P-wave)                 &                                              0.001 &                                              0.000 &                                              0.001 &                                              0.001 &                                              0.001 &                                              0.001 &                                              0.001 &                                              0.001 &                                              0.000 &                                              0.000 &                                              0.000 &                                              0.000 \\
$\mathcal{F}$($D_1(2600)$ P-wave)                 &                                              0.000 &                                              0.001 &                                              0.001 &                                              0.001 &                                              0.000 &                                              0.001 &                                              0.001 &                                              0.003 &                                              0.000 &                                              0.001 &                                              0.001 &                                              0.001 \\
$\mathcal{F}$($D_2(2740)$ P-wave)          &                                              0.000 &                                              0.000 &                                              0.000 &                                              0.000 &                                              0.000 &                                              0.000 &                                              0.000 &                                              0.000 &                                              0.000 &                                              0.000 &                                              0.000 &                                              0.000 \\
$\mathcal{F}$($D_2(2740)$ F-wave)          &                                              0.000 &                                              0.000 &                                              0.001 &                                              0.000 &                                              0.001 &                                              0.000 &                                              0.001 &                                              0.003 &                                              0.000 &                                              0.001 &                                              0.004 &                                              0.000 \\
\midrule
$D_{1}(2420)$ S-wave phase     &                                              0.010 &                                              0.024 &                                              0.029 &                                              0.031 &                                              0.005 &                                              0.012 &                                              0.017 &                                              0.036 &                                              0.012 &                                              0.004 &                                              0.004 &                                              0.012 \\
$D_{1}(2430)$ S-wave phase     &                                              0.003 &                                              0.002 &                                              0.007 &                                              0.007 &                                              0.005 &                                              0.005 &                                              0.009 &                                              0.046 &                                              0.007 &                                              0.005 &                                              0.001 &                                              0.006 \\
$D_{1}(2430)$ D-wave phase     &                                              0.017 &                                              0.015 &                                              0.027 &                                              0.027 &                                              0.016 &                                              0.004 &                                              0.045 &                                              0.042 &                                              0.003 &                                              0.028 &                                              0.076 &                                              0.004 \\
$D^{*}_{2}(2460)$ D-wave phase &                                              0.005 &                                              0.009 &                                              0.014 &                                              0.011 &                                              0.005 &                                              0.001 &                                              0.008 &                                              0.009 &                                              0.002 &                                              0.003 &                                              0.007 &                                              0.003 \\
$D_{0}(2550)$ P-wave phase     &                                              0.015 &                                              0.010 &                                              0.028 &                                              0.045 &                                              0.007 &                                              0.018 &                                              0.034 &                                              0.072 &                                              0.005 &                                              0.028 &                                              0.023 &                                              0.006 \\
$D^{*}_{1}(2600)$ P-wave phase &                                              0.006 &                                              0.005 &                                              0.013 &                                              0.017 &                                              0.018 &                                              0.016 &                                              0.014 &                                              0.026 &                                              0.001 &                                              0.012 &                                              0.014 &                                              0.002 \\
$D_{2}(2740)$ P-wave phase     &                                              0.014 &                                              0.008 &                                              0.038 &                                              0.030 &                                              0.030 &                                              0.041 &                                              0.070 &                                              0.107 &                                              0.014 &                                              0.019 &                                              0.061 &                                              0.019 \\
$D_{2}(2740)$ F-wave phase     &                                              0.010 &                                              0.007 &                                              0.022 &                                              0.017 &                                              0.016 &                                              0.012 &                                              0.024 &                                              0.054 &                                              0.003 &                                              0.032 &                                              0.030 &                                              0.005 \\
\end{tabular}

==> tables/unc2.tex <==
\begin{tabular}{l|rrrr|rrrr}
{} &  \begin{sideways}Normalis. sample size\end{sideways} &  \begin{sideways}Blatt-Weisskopf radius\end{sideways} &  \begin{sideways}Resonance parameters\end{sideways} &  \begin{sideways}Fit bias\end{sideways} &  \begin{sideways}Fitted value\end{sideways} &  \begin{sideways}Stat. uncert.\end{sideways} &  \begin{sideways}Total syst. uncert.\end{sideways} & \begin{sideways}Model uncert.\end{sideways} \\
\midrule
$D_1(2420)$ ${\rm Re}(c_{0,1})$       &                                              0.003 &                                              0.010 &                                              0.005 &                                   0.000 &                                      $-$0.088 &                                        0.033 &                                              0.018 &                           $-0.013$/$+0.029$ \\
$D_1(2420)$ ${\rm Im}(c_{0,1})$       &                                              0.003 &                                              0.012 &                                              0.004 &                                   0.000 &                                      $-$0.216 &                                        0.056 &                                              0.024 &                           $-0.046$/$+0.001$ \\
$D_1(2430)$ ${\rm Re}(c_{0,1})$       &                                              0.008 &                                              0.028 &                                              0.116 &                                   0.016 &                                       1.642 &                                        0.157 &                                              0.144 &                           $-0.202$/$+0.260$ \\
$D_1(2430)$ ${\rm Im}(c_{0,1})$       &                                              0.009 &                                              0.171 &                                              0.114 &                                   0.013 &                                       0.228 &                                        0.174 &                                              0.219 &                           $-0.285$/$+0.091$ \\
$D_1(2430)$ ${\rm Re}(c_{2,1})$       &                                              0.009 &                                              0.111 &                                              0.170 &                                   0.013 &                                      $-$0.325 &                                        0.261 &                                              0.217 &                           $-0.033$/$+0.213$ \\
$D_1(2430)$ ${\rm Im}(c_{2,1})$       &                                              0.007 &                                              0.257 &                                              0.298 &                                   0.003 &                                      $-$0.049 &                                        0.134 &                                              0.395 &                           $-0.046$/$+0.077$ \\
$D_2^*(2460)$ ${\rm Re}(c_{2,1})$     &                                              0.004 &                                              0.009 &                                              0.041 &                                   0.005 &                                      $-$0.641 &                                        0.045 &                                              0.045 &                           $-0.025$/$+0.020$ \\
$D_2^*(2460)$ ${\rm Im}(c_{2,1})$     &                                              0.003 &                                              0.053 &                                              0.071 &                                   0.007 &                                       0.002 &                                        0.071 &                                              0.090 &                           $-0.035$/$+0.027$ \\
$D_0(2550)$ ${\rm Re}(c_{1,1})$       &                                              0.003 &                                              0.018 &                                              0.033 &                                   0.004 &                                      $-$0.154 &                                        0.053 &                                              0.042 &                           $-0.053$/$+0.044$ \\
$D_0(2550)$ ${\rm Im}(c_{1,1})$       &                                              0.003 &                                              0.012 &                                              0.041 &                                   0.002 &                                      $-$0.194 &                                        0.052 &                                              0.048 &                           $-0.021$/$+0.110$ \\
$D_1^*(2600)$ ${\rm Re}(c_{1,1})$     &                                              0.003 &                                              0.013 &                                              0.066 &                                   0.008 &                                       0.528 &                                        0.066 &                                              0.070 &                           $-0.185$/$+0.013$ \\
$D_1^*(2600)$ ${\rm Im}(c_{1,1})$     &                                              0.003 &                                              0.048 &                                              0.065 &                                   0.020 &                                       0.175 &                                        0.089 &                                              0.088 &                           $-0.005$/$+0.234$ \\
$D_2(2740)$ ${\rm Re}(c_{1,1})$       &                                              0.001 &                                              0.007 &                                              0.015 &                                   0.007 &                                       0.153 &                                        0.065 &                                              0.021 &                           $-0.043$/$+0.033$ \\
$D_2(2740)$ ${\rm Im}(c_{1,1})$       &                                              0.001 &                                              0.004 &                                              0.018 &                                   0.007 &                                      $-$0.003 &                                        0.085 &                                              0.032 &                           $-0.073$/$+0.030$ \\
$D_2(2740)$ ${\rm Re}(c_{3,1})$       &                                              0.002 &                                              0.054 &                                              0.066 &                                   0.031 &                                       0.392 &                                        0.068 &                                              0.100 &                           $-0.006$/$+0.029$ \\
$D_2(2740)$ ${\rm Im}(c_{3,1})$       &                                              0.002 &                                              0.034 &                                              0.052 &                                   0.004 &                                      $-$0.036 &                                        0.107 &                                              0.069 &                           $-0.103$/$+0.032$ \\
\midrule
$\mathcal{F}$($D_1(2420)$ S-wave)          &                                              0.001 &                                              0.004 &                                              0.001 &                                   0.002 &                                       0.038 &                                        0.017 &                                              0.008 &                           $-0.001$/$+0.013$ \\
$\mathcal{F}$($D_1(2420)$ D-wave)          &                                              0.002 &                                              0.024 &                                              0.013 &                                   0.006 &                                       0.710 &                                        0.044 &                                              0.032 &                           $-0.060$/$+0.000$ \\
$\mathcal{F}$($D_1(2430)$ S-wave)          &                                              0.001 &                                              0.006 &                                              0.014 &                                   0.001 &                                       0.142 &                                        0.025 &                                              0.019 &                           $-0.020$/$+0.031$ \\
$\mathcal{F}$($D_1(2430)$ D-wave)          &                                              0.000 &                                              0.005 &                                              0.012 &                                   0.003 &                                       0.005 &                                        0.009 &                                              0.013 &                           $-0.005$/$+0.002$ \\
$\mathcal{F}$($D_2(2460)$ D-wave)                 &                                              0.001 &                                              0.001 &                                              0.002 &                                   0.002 &                                       0.117 &                                        0.014 &                                              0.005 &                           $-0.007$/$+0.000$ \\
$\mathcal{F}$($D_0(2550)$ P-wave)                 &                                              0.000 &                                              0.000 &                                              0.001 &                                   0.001 &                                       0.023 &                                        0.008 &                                              0.003 &                           $-0.017$/$+0.003$ \\
$\mathcal{F}$($D_1(2600)$ P-wave)                 &                                              0.000 &                                              0.005 &                                              0.003 &                                   0.001 &                                       0.048 &                                        0.010 &                                              0.007 &                           $-0.020$/$+0.011$ \\
$\mathcal{F}$($D_2(2740)$ P-wave)          &                                              0.000 &                                              0.000 &                                              0.000 &                                   0.002 &                                       0.004 &                                        0.004 &                                              0.002 &                           $-0.001$/$+0.001$ \\
$\mathcal{F}$($D_2(2740)$ F-wave)          &                                              0.000 &                                              0.006 &                                              0.002 &                                   0.001 &                                       0.023 &                                        0.007 &                                              0.008 &                           $-0.001$/$+0.004$ \\
\midrule
$D_{1}(2420)$ S-wave phase     &                                              0.011 &                                              0.040 &                                              0.018 &                                   0.001 &                                      $-$1.959 &                                        0.160 &                                              0.082 &                           $-0.053$/$+0.166$ \\
$D_{1}(2430)$ S-wave phase     &                                              0.005 &                                              0.103 &                                              0.054 &                                   0.009 &                                       0.138 &                                        0.105 &                                              0.127 &                           $-0.178$/$+0.059$ \\
$D_{1}(2430)$ D-wave phase     &                                              0.020 &                                              0.682 &                                              0.472 &                                   0.002 &                                      $-$2.992 &                                        0.419 &                                              0.837 &                           $-0.230$/$+0.551$ \\
$D^{*}_{2}(2460)$ D-wave phase &                                              0.005 &                                              0.083 &                                              0.111 &                                   0.011 &                                       3.138 &                                        0.110 &                                              0.141 &                           $-0.041$/$+0.053$ \\
$D_{0}(2550)$ P-wave phase     &                                              0.012 &                                              0.085 &                                              0.179 &                                   0.009 &                                      $-$2.242 &                                        0.214 &                                              0.225 &                           $-0.252$/$+0.049$ \\
$D^{*}_{1}(2600)$ P-wave phase &                                              0.006 &                                              0.078 &                                              0.108 &                                   0.031 &                                       0.319 &                                        0.156 &                                              0.145 &                           $-0.014$/$+0.371$ \\
$D_{2}(2740)$ P-wave phase     &                                              0.009 &                                              0.026 &                                              0.118 &                                   0.046 &                                      $-$0.022 &                                        0.558 &                                              0.207 &                           $-0.587$/$+0.163$ \\
$D_{2}(2740)$ F-wave phase     &                                              0.006 &                                              0.114 &                                              0.146 &                                   0.018 &                                      $-$0.091 &                                        0.270 &                                              0.204 &                           $-0.228$/$+0.082$ \\
\end{tabular}
